All Should Be Equal in the Eyes of Language Models: Counterfactually Aware Fair Text Generation

Fairness in Language Models (LMs) remains a longstanding challenge, given the inherent biases in training data that can be perpetuated by models and affect the downstream tasks. Recent methods employ expensive retraining or attempt debiasing during inference by constraining model outputs to contrast from a reference set of biased templates or exemplars. Regardless, they dont address the primary goal of fairness to maintain equitability across different demographic groups. In this work, we posit that inferencing LMs to generate unbiased output for one demographic under a context ensues from being aware of outputs for other demographics under the same context. To this end, we propose Counterfactually Aware Fair InferencE (CAFIE), a framework that dynamically compares the model understanding of diverse demographics to generate more equitable sentences. We conduct an extensive empirical evaluation using base LMs of varying sizes and across three diverse datasets and found that CAFIE outperforms strong baselines. CAFIE produces fairer text and strikes the best balance between fairness and language modeling capability

==> content/3-method-alt.tex <==
\section{Methodology}

In this section, we first formulate the problem and introduce relevant notations, and then delineate our framework \method that generates fair and unbiased outputs.  

\subsection{Task Formulation \incomplete}
\label{sec:prelim}

% LM related
Consider a pre-trained language model $\mathcal{M}$ with a finite vocabulary $\mathcal{V}$. Given a source context $C_{\text{source}}$ in the form of a sequence of tokens $x_1 \ldots x_{N}$, $\mathcal{M}$, generates a probability distribution $\mathbb{P}_{o}: \mathcal{V} \xrightarrow{} [0, 1]$. Based on the decoding strategy, $\mathbb{P}_{o}$ is then used to sample the next token $x_{N+1}$. The goal of this work is to ensure that the generated tokens produce an \textit{equitable} output without compromising the language modeling performance of $\mathcal{M}$. 

% Fairness Related
Sensitive attributes are the characteristics that are typically protected by ethical considerations and should not be used as the basis for making biased decisions. We denote a \textbf{sensitive attribute} as a set $\mathcal{A} = \{G_{1}, \ldots, G_{K} \}$ where $\mathcal{G}_{i}$ is a group comprising a set of \textbf{sensitive tokens} related to that \textbf{group} $\mathcal{G}_{i} = \{s_{1}, \ldots\}$. For instance, if the sensitive attribute is   ``religion", then the groups may be - {\textsc{Christianity}, \textsc{Church}, $\ldots$}, {\textsc{Judaism}, \textsc{Jewish} $\ldots$}, etc. Similarly, for the sensitive attribute  ``profession", the groups may be - {\textsc{Banker}}, {\textsc{CEO}}, {\textsc{Secretary}}, etc. In our work, we consider multiple sensitive attributes - gender, religion, race, and profession following~\cite{nadeem2020stereoset}.



\subsection{Debiasing with \method\incomplete}
\label{sec:method}

In this section, we present the \method, which given a language model and an input context produces continuations that exhibit \textit{equitability}. This means that the generated content does not display any bias towards or against any particular group $\textit{G}_{i}$ for all the sensitive attributes under consideration. Moreover, this equitable generation is achieved with minimal to negligible impact on the language modeling capability of the model. Our framework, \method first identifies sensitive tokens from the input context $C_{\text{source}}$. Next, \method creates counterfactual contexts by replacing the sensitive tokens identified in the previous step with their counterfactual tokens. \abhinav{Adding more here..}


\xhdr{\noindent{\textbf{Identifying Sensitive Tokens in $C_{\text{source}}$}}} 

\noindent To identify the sensitive tokens $s_{i}$ present in the source context $C_{\text{source}}$, we follow prior debiasing works~\cite{guo-etal-2022-auto, pennington-etal-2014-glove}. These works curate lists either manually or from the internet to incorporate sensitive words that may elicit gender and racial biases \abhinav{revise this line if necessary}. In this work, we create a more comprehensive list that encompasses a wider range of sensitive attributes including gender, race, religion, and profession. The details of the number and source of the word lists are supplied in the Appendix. We note that even though the extended list represents a significant improvement in the number of words, it is by no means exhaustive and holds potential for further expansion in future work. 

\xhdr{\noindent{\textbf{Creating Counterfactual Contexts}}} 
\noindent We then determine the group $\mathcal{G}_{i}$, that each sensitive token belongs to, and define a counterfactual token as an alternative sensitive token that is part of a different group. For instance, consider the sensitive token \textsc{church}, we sample sensitive tokens from other groups that act as counterfactuals, examples of these words may be \textsc{Judaism, Temple, Islam,} etc. 


Mathematically, we define the counterfactual of a given sensitive token $s_{\text{sensitive}} \in \mathcal{G}_{i}$ as:
\begin{equation}
     s_{\text{sensitive}}^{\prime} \in \mathcal{G}_j \quad \text{where} \quad \mathcal{G}_j \in \mathcal{A}, \, \mathcal{G}_j \neq \mathcal{G}_i
\end{equation}

where $s_{\text{sensitive}}^{\prime}$ is the counterfactual token and $\mathcal{G}_{j}$ is the group from which the counterfactual token is picked.

In this manner, we can obtain a list of $M$ counterfactual tokens, and construct $M$ counterfactual contexts $C_{\text{counterfactual}}$, by replacing source $s_{sensitive}$ with counterfactual $s_{\text{sensitive}}^{\prime}$. In the next step, we use these $M$ counterfactual contexts $C_{\text{counterfactual}}$ for adjusting the source context probability distribution.


\begin{figure}[ht!]
{
  \includegraphics[width=0.5\textwidth]{AnonymousSubmission/LaTeX/figures/BIAS ARCHITECTURE.pdf}%
%\vspace{-18pt}
}
\caption{A demonstration of the CAFIE algorithm: Utilizing a base language model (LM) to process input sentences with a target group and $m$ counterfactual groups. Our approach identifies sensitive counterfactual groups, modifies probability distributions to mitigate influence from alternate groups, and yields a probability distribution that encapsulates both the original and counterfactual perspectives
}
\label{fig:architecture}
\end{figure}


\xhdr{\noindent{\textbf{Step 3: Calibrating $\mathbb{P}_{0}$}} with Disparity Score ($\Delta_{k}$)}

% When using a language model $\mathcal{L}$, it generates a next-token probability distribution based on an input context. Given the biases these models might have inherited during training, we propose to use counterfactual contexts to recalibrate and refine these probabilities.

% The initial step is for the model to generate next-token probabilities for the original context, denoted as $\mathbb{P}{0}$, and for each counterfactual context, represented as $\mathbb{P}{1}, \ldots, \mathbb{P}_{m}$. 

\noindent We generate the probability distributions used for sampling the next token for our source context $C_{\text{source}}$ and the counterfactual contexts $C^{1}, \ldots, C^{M-1}$. We denote these distributions as $\mathbb{P}_{0}, \ldots, \mathbb{P}_{M-1}$. We then compute a disparity score ($\Delta_{k}$) which compares the difference in next-token probability distributions of the input context ($\mathbb{P}_{0}$) and a counterfactual context ($\mathbb{P}_{k}$), where $k \in [1, M-1]$. With this score, we establish that 

% In language models, biases manifest as uneven probability distributions for sensitive attributes in certain contexts. For this, our approach first computes a disparity score ($\Delta_{k}$) which compares difference in next-token probability distributions of the input context ($\mathbb{P}_{0}$) and a counterfactual context ($\mathbb{P}_{k}$), where $k \in m$ counterfactuals. With this score, \method establishes for what tokens does language model $\mathcal{L}$ associates the input context's sensitive token $\mathbb{P}_{0}$ with and does not associate with the counterfactual context's sensitive token, thereby, highlighting the biases. 


\begin{equation}
\begin{aligned}
\Delta_{k} &= \mathbb{P}_{0} - \mathbb{P}_{k}, \\
\end{aligned}\label{disparity}
\end{equation}

% 
%$c^{1} \ldots c^{m}$, \method compares them with input context $c$, 
%and generates $m+1$ probability distributions $\mathbb{P}_{0}, \mathbb{P}_{1}, \ldots, \mathbb{P}_{m}$ from $\mathcal{L}$. 
%Each $\mathbb{P}_{k}$ conveys vital information about the biases of $\mathcal{L}$ for the $k^{th}$ group. 

% By recalibrating the original probability distribution using the information from the counterfactual distributions, we can improve the fairness of the text generation. 

% Specifically, we compare the probability distribution of the original input with the distributions generated for the counterfactuals and use this information to adjust the original distribution. The weights for this transformation are computed as -


\noindent\textbf{Step 4: Weighing the Disparity with $\mathbf{W}_{k}$:}
\surgan{meaning of first line is not clear to me. For a given context, and input, which are the different tokens here}
\noindent For a given pair of counterfactual and input context, the disparity scores vary for different tokens. Intuitively, the larger the disparity between original and a counterfactual, the greater the necessity to adjust the original probabilities to counteract inherent biases. \surgan{our ablation results over function suggest that tanh is better than sigmoid. even sigmoid might be interpretable. so there are things beyond interpretability. we can avoid for reviewer's brows} To make the scores more interpretable, we use $\tanh$ and scale the scores to the range [-1, 1]. And further control the sensitivity of the adjustments, we make use of $\lambda$. We add 1 to the equation to account for cases with the absence of disparity (unbiased words like stop-words) and ensure the original probabilities remain unaffected.

%In-case of no disparities ($\Delta_{k}=0$), for example, for stop-words continuations, 
%We use a $-1 \times  \times \Delta_{k}$ for controlling the sensitivity of the calibration of probabilities in the next step. 

\begin{equation}
\begin{aligned}
\mathbf{W}_{k} &= \mathrm{tanh}(-\lambda \Delta_{k}) + 1
\end{aligned}
\end{equation}

%where $\Delta_{k}$ are is the disparity score, $\mathbf{W}_{k}$ are the adjustment weights, $\lambda$ is a hyperparameter, and $\mathbb{P}_{0}, \mathbb{P}_{k}$ are the probability of the original input and the $k^{th}$ counterfactual respectively. 

\noindent\textbf{Step 5: Counterfactual-Informed adjusted distribution:}
\noindent Finally, for a holistic and balanced calibration, we compute a weighted sum for every counterfactual and input context, where $\mathbf{W}_{k}$ is proportional to the individual disparities. This ensures that the biases from the original input context are adequately counterbalanced by the biases gathered from the different counterfactuals.
\begin{equation}
\begin{aligned}
\mathbb{P_{\text{\textbf{C-Informed}}}} = \sum_{i=1}^{M} \frac {e^{|\Delta_{i}|}} {\sum_{j=1}^{M} e^{|\Delta_{j}|}} \mathbf{W}_{i} \mathbb{P}_{0}
\end{aligned}
\end{equation}

\surgan{double mod to mod}
% $\tilde{\mathbb{P}}$

where $\mathbb{P_{\text{\textbf{C-Informed}}}}$ is the counterfactual-aware distribution. 

%recalibrate the original probability by weighing with individual . 
%To converge to an adjusted probability distribution that accounts for biases across all counterfactuals, we employ a weighted sum.
%We obtain the final updated probabilities by taking a weighted sum of $\mathbf{W}_{k}$'s based on their disparity score $\Delta_{k}$ and multiply it with $\mathbb{P}_{0}$ as -

\subsection*{Step 6: Fair Decoding with Counterfactual Aware Distribution}
\noindent While the counterfactual-informed adjusted distribution ensures equitability across counterfactuals, the essence of original context must be retained. To address this, we  compute the following linear combination between original input context distribution $\mathbb{P}_{0}$ and the counterfactual-informed adjusted distribution $\mathbb{P_{\text{\textbf{C-Informed}}}}$ and produce unbiased text and relevant to the actual input.

%While $\tilde{\mathbb{P}}$ does produce equitable outputs across $M$ counterfactual demographics, the final outputs should retain the context of the actual input $c$. Therefore, we compute the final probabilities as the linear combination of $\tilde{\mathbb{P}}$ and $\mathbb{P}_{0}$ as -

\begin{equation}
\mathbb{P_{\textbf{\text{FAIR}}}} = \alpha \mathbb{P_{\text{\textbf{C-Informed}}}} + (1-\alpha) \mathbb{P}_{0}
\end{equation}

where $\mathbb{P_{\textbf{\text{FAIR}}}}$ is the fair probability distribution that we sample the next token from, and $\alpha$ is a hyperparameter.

